Addressing Data Heterogeneity in Decentralized Learning via Topological Pre-processing

Recently, local peer topology has been shown to influence the overall convergence of decentralized learning (DL) graphs in the presence of data heterogeneity. In this paper, we demonstrate the advantages of constructing a proxy-based locally heterogeneous DL topology to enhance convergence and maintain data privacy. In particular, we propose a novel peer clumping strategy to efficiently cluster peers before arranging them in a final training graph. By showing how locally heterogeneous graphs outperform locally homogeneous graphs of similar size and from the same global data distribution, we present a strong case for topological pre-processing. Moreover, we demonstrate the scalability of our approach by showing how the proposed topological pre-processing overhead remains small in large graphs while the performance gains get even more pronounced. Furthermore, we show the robustness of our approach in the presence of network partitions.

==> Arxiv/08_supplementary_materials.tex <==
\newpage
\onecolumn
\section{\centering{Supplementary experimental results}}

\label{sec:sup}


\subsection{Summary}
In supplementary materials, we also exhibit the situation where \proj is not outperform baselines. This is reasonable, since every method have their own strength and weakness, there is no superior solution can universal in all possible FL settings.
Again, we summarized scenarios that \proj shows in advanced: 
1. bandwidth matters.
2. public data available  
3. edge devices are resource limited.
4. large scale.

\subsection{Learning Efficiency}

\subsection{Communication Cost}

\subsection{Ablation Study}

\subsection{Difference}


==> Arxiv/figtex/network_updates.tex <==
\begin{figure}%
    \centering
    \subfloat[\centering Server ensembles students for KD.]{{\includegraphics[width=0.4\linewidth]{Figures/FL_KD_global.png} }}%
    \qquad
    \subfloat[\centering Client's use DML to train their student.]{{\includegraphics[width=0.4\linewidth]{Figures/FL_KD_local.png} }}%
    \caption{The server ensembles uploaded students to generate soft labels for a public unlabeled dataset.
The soft-labels and unlabeled data are then used to train the global student before it gets downloaded.}%
    \label{fig:example}%
\end{figure}

==> Arxiv/figtex/overview.tex <==
\begin{figure*}%
    \centering
    \includegraphics[width=\linewidth]{Arxiv/Figures/overview_v3.pdf}
    \caption{During initialization, edge clients request for a customized neural architecture and a student model. During local training, the client's customized subnetwork and student network are trained in tandem. The server uses ensemble learning to distill global knowledge.  }%
    \label{fig:overview}%
\end{figure*}
